Synthesis and Verification of Transformer Programs (Technical Report)

C-RASP is a simple programming language that was recently shown to capture concepts expressible by transformers. In this paper, we develop new algorithmic techniques for automatically verifying C-RASPs. To this end, we establish a connection to the verification of synchronous dataflow programs in Lustre, which enables us to exploit state-of-the-art model checkers utilizing highly optimized SMT-solvers. Our second contribution addresses learning a C-RASP program in the first place. To this end, we provide a new algorithm for learning a C-RASP from examples using local search. We demonstrate efficacy of our implementation for benchmarks of C-RASPs in the literature, in particular in connection to the following applications: (1) transformer program optimization, and (2) constrained learning of transformer programs (based on a partial specification).

==> app/language.tex <==
\section{Benchmark Languages and C-RASP Constructions}
\label{app:benchmark-table}

\paragraph{Dyck-1} is the language of well-balanced parentheses over
$\Sigma=\{l,r\}$: every prefix contains at least as many $l$ as $r$, and the
total numbers of $l$ and $r$ are equal.


\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for Dyck-\(1\) over \(\Sigma=\{l,r\}\)},
	center
	]
	\[
	\begin{aligned}
		L  &= l\\
		R &= r\\
		V &= CL < CR\\
		M &= CV = C0\\
		B &= CL = CR\\
		Out &= M \land B\\
		CL &= \#l\\
		CR &= \#r\\
		CV &= \#V\\
		C0 &= 0
	\end{aligned}
	\]
\end{tcolorbox}
\paragraph{a$^*$b$^*$} is the language of strings over $\Sigma=\{a,b\}$ consisting of a block
of $a$'s followed by a block of $b$'s (possibly empty blocks).

\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for $a^*b^*$  over \(\Sigma=\{l,r\}\)},
	center
	]
	\[
	\begin{aligned}
		Qa &= a\\
		Qb &= b\\
		V  &= Qa \land (0 < Cb) \\    
		Y  &= CV = 0             \\
		Cb &= \#Qb\\               
		CV &= \#V    \\   
		Out &= Y  
	\end{aligned}
	\]
\end{tcolorbox}

\paragraph{MAJORITY} is the language of strings over $\Sigma=\{a,b\}$ with at least
as many $a$ symbols as $b$ symbols.

\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for Majority over \(\Sigma=\{a,b\}\)},
	center
	]
	\[
	\begin{aligned}		
		Pa &= a\\
		Pb &= b\\
		Out &= Ca \leq Cb\\
		Ca &= \#Pa\\
		Cb &= \#Pb\\
	\end{aligned}
	\]
\end{tcolorbox}

\paragraph{(aa)$^*$} is the language of even-length strings over $\Sigma=\{a\}$.



\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for $(aa)^*$ over \(\Sigma=\{a\}\)},
	center
	]
	\[
	\begin{aligned}		
		CnotA &= \#(\neg a) \\
		Out &= (\%2=1) \land (CnotA=0)
	\end{aligned}
	\]
\end{tcolorbox}


\paragraph{a$^n$b$^n$c$^n$} is the language $\{a^n b^n c^n \mid n\ge 0\}$ over $\Sigma=\{a,b,c\}$.

 
\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for $a^nb^nc^n$ over \(\Sigma=\{a, b, c\}\)},
	center
	]
	\[
	\begin{aligned}		
		Qa &= a\\
		Qb &= b\\
		Qc &= c\\
		Ca &= \#Qa\\
		Cb &= \#Qb\\
		Cc &= \#Qc\\
		A  &= Cb + Cc = 0\\
		B  &= Cc = 0\\
		QaA &= Qa \land A\\
		QbB &= Qb \land B\\
		CA &= \#QaA\\
		CB &= \#QbB\\
		Ga &= CA = Ca\\
		Gb &= CB = Cb\\
		Gabc &= (Ca = Cb) \land (Cb = Cc)\\
		Out &= Ga \land Gb \land Gabc
	\end{aligned}
	\]
\end{tcolorbox}

\paragraph{$\Sigma^*$ab$\Sigma^*$}over $\Sigma=\{a,b\}$ is the language of strings containing
the substring $ab$ at some position.


\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for $\Sigma^*$ab$\Sigma^*$  over \(\Sigma=\{a, b\}\)},
	center
	]
	\[
	\begin{aligned}		
		CaPre &= \#<(1) a\\
		PaPre &= 1 \leq CaPre\\
		Qab &= b \land PaPre\\
		Cab &= \#Qab\\
		Out &= 1 \leq Cab
	\end{aligned}
	\]
\end{tcolorbox}

 


\paragraph{Existential} is the language of strings over $\Sigma=\{a,b\}$ containing
at least one occurrence of $a$.

\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for Existential over \(\Sigma=\{a,b\}\)},
	center
	]
	\[
	\begin{aligned}		
		A &= a \\
		B &= b \\
		C1 &= \#A \\ 
		C2 &= \#B \\ 
		Out &= 1 <= C2
	\end{aligned}
	\]
\end{tcolorbox}


\paragraph{Next(Argmax)} is the language over $\Sigma$ in which, for each position
$i>1$, the observed successor $x_i$ maximises (ties allowed) the empirical
count of transitions from the previous symbol $x_{i-1}$, compared against all
alternative successors $c\in\Sigma$, using statistics computed from the prefix
up to position $i-1$.



\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for Next(Argmax) over \(\Sigma=\{a, b, c\}\)},
	center
	]
	\[
	\begin{aligned}		
		C1 &= \#(1,1) a\\
		B1 &= 1 \leq C1\\
		B2 &= a \land B1\\
		B3 &= b \land B1\\
		B4 &= c \land B1\\
		C2 &= \#B2\\
		C3 &= \#B3\\
		C4 &= \#B4\\
		B5 &= C3 \leq C2\\
		B6 &= C4 \leq C2\\
		B7 &= 1 \leq (C2 + C3 + C4)\\
		B8 &= a \land B7 \land B5 \land B6\\
		Out &= 1 \leq \#B8
	\end{aligned}
	\]
\end{tcolorbox}



\paragraph{Tomita 1} is the regular language $a^*$ over $\Sigma=\{a,b\}$, i.e.,
strings containing no occurrences of $b$.


\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for Tomita 1 over \(\Sigma=\{a, b\}\)},
	center
	]
	\[
	\begin{aligned}		
		B1 &= b \\
		C1 &= \#B1 \\
		Out &= (C1 = 0)
	\end{aligned}
	\]
\end{tcolorbox}

\paragraph{Tomita 2} is the regular language $(ab)^*$ over $\Sigma=\{a,b\}$, i.e.,
strings of even length that alternate starting with $a$ and ending with $b$.


\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for Tomita 2 over \(\Sigma=\{a, b\}\)},
	center
	]
	\[
	\begin{aligned}		
		B1 &= (a \land \%2=0) \lor (b \land \%2=1)\\
		B2  &= \#(\neg B1)\\
		Out &= (\%2=1) \land (B2 = 0)
	\end{aligned}
	\]
\end{tcolorbox}

\paragraph{Tomita 4} is the regular language over $\Sigma=\{a,b\}$ that forbids any
substring of the form $a\,b^{2n+1}\,a^{2m+1}\,b$ for $n,m\ge 0$.
Equivalently, $w \in \textsc{Tomita-4}$ iff no occurrence of $a$ is followed by
an odd run of $b$'s, then an odd run of $a$'s, and then a $b$.

\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for Tomita 4 over \(\Sigma=\{a, b\}\)},
	center
	]
	\[
	\begin{aligned}		
		A1 &= \#(1,1) a\\
		P1 &= 1 \leq A1\\
		A2 &= \#(2,2) a\\
		P2 &= 1 \leq A2\\
		AAApos &= a \land P1 \land P2\\
		CAAA &= \#AAApos\\
		Out &= (CAAA = 0)
	\end{aligned}
	\]
\end{tcolorbox}

\paragraph{Tomita 7} is the regular language $a^*b^*a^*b^*$ over $\Sigma=\{a,b\}$,
i.e., strings that can be partitioned into at most four consecutive blocks,
alternating between $a$'s and $b$'s starting with $a$.
\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for Tomita 7 over \(\Sigma=\{a, b\}\)},
	center
	]
	\[
	\begin{aligned}		
		B &= b\\
		A &= a\\
		Cb    &= \#B\\
		B1 &= 1 \leq Cb\\
		B2 &= A \land B1\\
		C1  &= \#B2\\
		B3 &= 1 \leq C1\\
		B4 &= B \land B3\\
		CBAB            &= \#B4\\
		B1AB          &= 1 \leq CBAB\\
		B5 &= A \land B1AB\\
		CBadA   &= \#B5\\
		Out &= (CBadA = 0)
	\end{aligned}
	\]
\end{tcolorbox}



\paragraph{PT-5} is the piecewise testable language over $\Sigma=\{a,b,c,d,e\}$ in
which $a,b,c,d,e$ occur in this order as a (not necessarily contiguous)
subsequence. Formally, $w \in \textsc{PT-5}$ iff there exist
$i_1<i_2<i_3<i_4<i_5$ with $w[i_1]=a$, $w[i_2]=b$, $w[i_3]=c$, $w[i_4]=d$,
and $w[i_5]=e$.

\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for PT-5 over \(\Sigma=\{a, b, c, d, e\}\)},
	center
	]
	\[
	\begin{aligned}		
		A &= a\\
		B &= b\\
		C &= c\\
		D &= d\\
		E &= e\\
		CA &= \#A\\
		L1 &= 1 <= CA\\
		QB &= B \land  L1\\
		CB &= \#QB\\
		L2 &= 1 \leq CB\\
		QC &= C \land  L2\\
		CC &= \#QC\\
		L3 &= 1 \leq CC\\
		QD &= D \land L3\\
		CD &= \#QD\\
		L4 &= 1 \leq CD\\
		QE &= E \land  L4\\
		CE &= \#QE\\
		L5 &= 1 \leq CE\\
		Out &= L5
	\end{aligned}
	\]
\end{tcolorbox}



\paragraph{PT-3} over $\Sigma=\{a,b,c\}$ in which
$a$, then $b$, then $c$ occur in this order (not necessarily consecutively).
Formally, $w \in \textsc{PT-3}$ iff there exist indices $i<j<k$ such that
$w[i]=a$, $w[j]=b$, and $w[k]=c$.

\begin{tcolorbox}[
	enhanced,
	width=1\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for PT-3 over \(\Sigma=\{a, b, c\}\)},
	center
	]
	\[
	\begin{aligned}		
		A &= a\\
		B &= b\\
		C &= c\\
		CA &= \#A\\
		L1 &= 1 \leq CA\\
		QB &= B \land  L1\\
		CB &= \#QB\\
		L2 &= 1 \leq CB\\ 
		QC &= C \land  L2\\
		CC &= \#QC\\
		L3 &= 1 \leq CC\\  
		Out &= L3
	\end{aligned}
	\]
\end{tcolorbox}






\paragraph{PT-2}  over $\Sigma=\{a,b\}$
	consists of strings in which an $a$ occurs before some later $b$.

\begin{tcolorbox}[
	enhanced,
	width=\linewidth,
	colback=gray!8,
	colframe=black,
	boxrule=0.6pt,
	arc=2pt,
	left=6pt,
	right=6pt,
	top=4pt,
	bottom=4pt,
	title={\(C\)-RASP program for PT-2 over \(\Sigma=\{a, b\}\)},
	center
	]
	\[
	\begin{aligned}		
		A &= a\\
		B &= b\\
		CA &= \#A\\
		L1 &= 1 \leq CA\\
		QB &= B \land L1\\
		CB &= \#QB\\
		L2 &= 1 \leq CB \\
		Out &= L2
	\end{aligned}
	\]
\end{tcolorbox}
 

==> app/lustreapp.tex <==
\subsection{Additional Definitions for Lustre}

\subsubsection{Definition of Expression Evaluation}

We define $\lval(e, i)$ in full for Lustre expressions.
For Boolean expressions
\[
    \begin{aligned}
        \lval(\top, i) &= \top \\
        \lval(\bot, i) &= \bot \\
        \lval(\neg e, i) &= \neg \lval(e, i) \\
        \lval(e_1 \diamond_b e_2, i)
             &= \lval(e_1, i) \diamond_b \lval(e_2, i) \\
        \lval(e_1 \bowtie_b, i)
             &= \lval(e_1, i) \bowtie_b \lval(e_2, i) \\
        \lval(\lpre(e), i) &= \begin{cases}
            \lval(e, i - 1) & \text{when $i > 0$} \\
            \text{undefined} & \text{otherwise}
        \end{cases} \\
        \lval(e_1 \lnext e_2, i) &= \begin{cases}
                \lval(e_1, i) & \text{if $i = 0$} \\
                \lval(e_2, i) & \text{otherwise}
            \end{cases}
    \end{aligned}
\]
and for integer expressions
\[
    \begin{aligned}
        \lval(k, i) &= k \\
        \lval(e_1 \diamond_c e_2, i)
            &= \lval(e_1, i) \diamond_c \lval(e_2, i) \\
        \lval(\lif e_1 \lthen e_2 \lelse e_3, i) &= \begin{cases}
            \lval(e_2, i) & \text{if $\lval(e_1, i) = \top$} \\
            \lval(e_3, i) & \text{otherwise} \\
        \end{cases} \\
        \lval(\lpre(e), i) &= \lval(e, i - 1) \\
        \lval(e_1 \lnext e_2, i) &= \begin{cases}
                \lval(e_1, i) & \text{if $i = 0$} \\
                \lval(e_2, i) & \text{otherwise.}
            \end{cases}
    \end{aligned}
\]

\subsubsection{Translating C-RASP to Lustre}

We define $T(e)$ in full.
For Boolean expressions (recalling that $I = a$ denotes $I = \latoi(a)$)
\[
    \begin{aligned}
        T(\top) & \ldef \top \\
        T(\bot) & \ldef \bot \\
        T(a) & \ldef I = a \\
        T(B) & \ldef V_B \\
        T(\neg e) & \ldef \neg T(e) \\
        T(e_1 \diamond e_2) & \ldef T(e_1) \diamond T(e_2) \\
        T(e_1 \bowtie e_2) & \ldef T(e_1) \bowtie T(e_2) \\
        T(m\%o) & \ldef P \lmod m = o \\
    \end{aligned}
\]
where $P$ is a fresh integer variable encoding the current position.
It uses an auxiliary equation $P \ldef 0 \lnext \lpre(P) + 1$.
For counting expressions
\[
    \begin{aligned}
        T(k) & \ldef k \\
        T(C) & \ldef V_C \\
        T(\#(e)) & \ldef C_{\#(e)} \\
        T(\#_{r_s, r_e}(e)) & \ldef C_{\#_{r_s, r_e}(e)} \\
        T(e_1 + e_2) & \ldef T(e_1) + T(e_2) \\
        T(e_1 - e_2) & \ldef T(e_1) - T(e_2) \\
        T(\min(e_1, e_2)) & \ldef
            \lif C_{e_1} < C_{e_2} \lthen C_{e_1} \lelse C_{e_2} \\
        T(\max(e_1, e_2)) & \ldef
            \lif C_{e_2} < C_{e_1} \lthen C_{e_1} \lelse C_{e_2} \\
        T(e_1\ ?\ e_2\ :\ e_3) & \ldef
            \lif T(e_1) \lthen T(e_2) \lelse T(e_3) \\
    \end{aligned}
\]
where $C_{\#(e)}$, $C_{\#_{r_s, r_e}(e)}$, $C_{e_1}$, and $C_{e_2}$ are fresh
integer variables defined via the auxiliary equations.

The additional auxiliary equations are: for each $C_{e_i}$ add the rule
\[
    C_{e_i} \ldef T(e_i).
\]

\subsubsection{Additional Verification Properties}

\paragraph{Universality}

Let $P = (R_1, \ldots, R_k)$ be a C-RASP program.
Universality can be checked by inspecting the value of $R_k = B \ldef e$
(corresponding to the final C-RASP rule).
For universality, we require that $R_k$ always evaluates to $\top$.
It requires the following $\lcheck$ constraint which asserts that after the
first position, either the input $I$ is incorrect, the end of the stream marker
has not been reached, or the value of $R_k$ is $\top$.
\[
    \lcheck \top \lnext (\neg(B_{\hat{I}} \land I = \leos) \lor \lpre(V_B))
\]

We define $\tvalid(P)$ to be the Lustre program with the equations $\mathcal{R}_I
\cup \bigcup_i T(R_i)$ and the check statement defined above.

\begin{proposition}
    A C-RASP program $P$ accepts all words $w \in \Sigma^+$ if $\tvalid(P)$ is
    valid.
\end{proposition}

\paragraph{Language Equality}
We can check the equivalence of two C-RASP programs $P_1$ and $P_2$ using a similar encoding to language inclusion.
We need to adjust the $\lcheck$ equation as shown below.
\[
    \lcheck \top \lnext \left(
        \begin{array}{c}
            \neg(B_{\hat{I}} \land I = \leos) \\
            \lor\ (\lpre(V_1) \land \lpre(V_2)) \\
            \lor\ (\neg \lpre(V_1) \land \neg \lpre(V_2))
        \end{array}
    \right)
\]

We define $\tequal(P_1, P_w)$ to be the Lustre program with the equations
$\mathcal{R}_I \cup \bigcup_i T(R^1_i) \cup \bigcup_i T(R^2_i)$ and the check
statement defined above.

\begin{proposition}
    A C-RASP program $P_1$ accepts the same words $w \in \Sigma^+$ accepted by a
    C-RASP program $P_2$ if $\tequal(P_1, P_2)$ is valid.
\end{proposition}




==> intro.tex <==
% speak about transformers
Transformers are the underlying neural network architectures behind Large
Language Models (LLMs). In contrast to Recurrent Neural Networks \cite{?} --- 
which sequentially process the input sequence from left to right ---
transformers use attention to aggregate the input sequence with respect to each
position \cite{Vaswani17}. Among others, this results in a neural model that 
is quite expressive \cite{?}, but is efficiently parallelizable \cite{?}.
Despite these, transformers are in general quite tricky to analyze \cite{?}.
Say about undecidability and Turing-completeness.

% speak about RASP and C-RASPs
To better understand the behavior of transformers, researchers proposed to
develop declarative languages which enjoy precisely defined semantics and at the
same time faithfully capture the behavior of transformers. In 2021 Weiss et al.
\cite{weiss2021thinking} proposed the influential RASP (Restricted Access
Sequence Processing Language) paradigm for such a declarative language.
Essentially, RASP is a programming language that operates on sequences via
operations like selection, aggregation, and simple position-wise arithmetic 
operations. Over the years the RASP paradigm has been instantiated and formally
proven to be specific classes of transformers. The simplest RASP is B-RASP
(Boolean RASP), which supports manipulations of sequences of 0s and 1s. This
language was also proven to be equivalent to Linear Temporal Logic, which is
equivalent to a subset of regular expressions called star-free regular
expressions. 

